WildGait: Learning Gait Representations from Raw Surveillance Streams

The use of gait for person identification has important advantages such as being non-invasive, unobtrusive, not requiring cooperation and being less likely to be obscured compared to other biometrics. Existing methods for gait recognition require cooperative gait scenarios, in which a single person is walking multiple times in a straight line in front of a camera. We aim to address the challenges of real-world scenarios in which camera feeds capture multiple people, who in most cases pass in front of the camera only once. We address privacy concerns by using only motion information of walking individuals, with no identifiable appearance-based information. As such, we propose a novel weakly supervised learning framework, WildGait, which consists of training a Spatio-Temporal Graph Convolutional Network on a large number of automatically annotated skeleton sequences obtained from raw, real-world, surveillance streams to learn useful gait signatures. We collected the training data and compiled the largest dataset of walking skeletons called Uncooperative Wild Gait, containing over 38k tracklets of anonymized walking 2D skeletons. We release the dataset for public use. Our results show that, with fine-tuning, we surpass the current state-of-the-art pose-based gait recognition solutions. Our proposed method is reliable in training gait recognition methods in unconstrained environments, especially in settings with scarce amounts of annotated data.

==> sections/tabels/other.tex <==

% \setlength{\tabcolsep}{0.9em}
% {\renewcommand{\arraystretch}{1.2}
% \begin{table}[hbt!]
%     \centering
%     \begin{tabular}{l | c}
%         \textbf{Method} &  \textbf{CASIA-B Mean Acc.}\\
%         \hline\hline
%          ST-GCN + Random Cropping & 60.8 \% \\
%          + Squeeze \& Flip & 64.6 \% \\
%          + Random Pace &  61.3 \%\\
%          + Sequence Shuffle & \textbf{68.0 \%} \\
%         %  + Label Smoothing & 62.3 \%
%     \end{tabular}
%     \caption{Accuracy improvements of each augmentation scheme. {\color{red} TODO needs re-evaluation?}}
%     %\caption{Ablation results on the various augmentation schemes we used. {\color{red} TODO needs re-evaluation?}}
%     \label{tab:ablation}
% \end{table}
% }

% \setlength{\tabcolsep}{0.8em}
% {\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
%     \resizebox{\textwidth}{!}{
%     \centering
%     \begin{tabular}{l | rrrrrrrrrrr| r}
%     \toprule
%         \textbf{Method} &  0$^{\circ}$  &    18$^{\circ}$  &    36$^{\circ}$  &    54$^{\circ}$  &    72$^{\circ}$  &    90$^{\circ}$  &    108$^{\circ}$ &    126$^{\circ}$ &   144$^{\circ}$ &    162$^{\circ}$ &    180$^{\circ}$ & Mean \\
%         \midrule
%         Pretrain Kinetics  & 19.35 &  19.35 &  27.42 &  29.03 &  25.81 &  38.71 &  27.42 &  27.42 &  20.97 &  12.9 &  6.45 &  23.17 \\
%         \hline
%         Predict \& Cluster & 32.26 &  42.74 &  44.35 &  31.45 &  29.03 &  48.39 &  44.35 &  43.55 &  29.03 &  16.94 &  16.94 &  34.46 \\
%         \hline
%         MS$^2$L & 32.26 &  36.29 &  47.58 &  41.13 &  21.77 &  44.35 &  47.58 &  49.19 &  37.9 &  23.39 &  19.35 &  36.44 \\
%         Pace Pred.  & 42.34 &  63.31 &  70.56 &  56.05 &  52.02 &  62.5 &  62.1 & \textbf{ 74.19} &  \textbf{67.74} &  37.5 &  45.97 &  57.66 \\
%         \hline
%         WildGait \textbf{(ours)} & \textbf{58.06} &  \textbf{74.19} &  \textbf{83.06} &  \textbf{74.19} &  \textbf{60.48} &  \textbf{75.81} &  \textbf{74.19} &  \textbf{74.19} &  65.32 &  \textbf{54.03} &  \textbf{54.84} &  \textbf{68.04} \\
%     \end{tabular}}
%     \caption{Transfer learning comparison with other unsupervised skeleton-based training methods.}
%     \label{tab:unsupervised}
% \end{table*}
% }


% \setlength{\tabcolsep}{0.8em}
% {\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
%     \resizebox{\textwidth}{!}{
%     \centering
%     \begin{tabular}{l | rrrrrrrrrrr| r}
%     \toprule
%         \textbf{Method} &  0$^{\circ}$  &    18$^{\circ}$  &    36$^{\circ}$  &    54$^{\circ}$  &    72$^{\circ}$  &    90$^{\circ}$  &    108$^{\circ}$ &    126$^{\circ}$ &   144$^{\circ}$ &    162$^{\circ}$ &    180$^{\circ}$ & Mean \\
%         \midrule
%         Pretrain Kinetics \cite{yan2018spatial} & \textbf{10.48} &  7.26 &  6.45 &  12.9 &  1.61 &  12.1 &  16.94 &  18.55 &  11.29 &  4.03 &  3.23 &  9.53 \\
%         \hline
%         Predict \& Cluster \cite{su2019predict} & 12.9 & \textbf{ 20.16} &  \textbf{21.77} &  \textbf{18.55} &  8.06 &  16.13 &  13.71 &  17.74 &  8.06 &  7.26 &  8.87 &  13.93 \\
%         \hline
%         MS$^2$L \cite{Lin_2020} & 3.23 &  8.87 &  10.48 &  8.87 &  6.45 &  9.68 &  18.55 &  21.77 &  11.29 &  7.26 &  9.68 &  10.56 \\
%         Pace Pred. \cite{wang2020selfsupervised} & 9.27 &  12.1 &  13.31 &  12.1 &  9.27 &  12.1 &  14.11 &  21.37 &  14.11 &  10.48 &  9.68 &  12.54 \\
%         \hline
%         WildGait \textbf{(ours)}  & \textbf{10.48} &  19.35 &  14.52 &  13.71 & \textbf{ 10.48} &  \textbf{16.94} &  \textbf{20.16} &  \textbf{25.0} & \textbf{ 17.74} & \textbf{ 19.35} &  \textbf{12.9} &  \textbf{16.42} \\
%     \end{tabular}}
%     \caption{Experiment B.}
%     \label{tab:unsupervised-casia-clothing}
% \end{table*}
% }

% \setlength{\tabcolsep}{0.8em}
% {\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
%     \resizebox{\textwidth}{!}{
%     \centering
%     \begin{tabular}{l | rrrrrrrrrrr| r}
%     \toprule
%         \textbf{Method} &  0$^{\circ}$  &    18$^{\circ}$  &    36$^{\circ}$  &    54$^{\circ}$  &    72$^{\circ}$  &    90$^{\circ}$  &    108$^{\circ}$ &    126$^{\circ}$ &   144$^{\circ}$ &    162$^{\circ}$ &    180$^{\circ}$ & Mean \\
%         \midrule
%         Pretrain Kinetics \cite{yan2018spatial}&  16.13 &  20.16 &  13.71 &  19.35 &  7.26 &  15.32 &  12.9 &  15.32 &  11.29 &  6.45 &  5.65 &  13.05 \\
%         \hline
%         Predict \& Cluster \cite{su2019predict} &  25.0 &  25.81 &  29.84 &  25.0 &  18.55 &  21.77 &  25.81 &  24.19 &  17.74 &  13.71 &  12.1 &  21.77 \\
%         \hline
%         MS$^2$L \cite{Lin_2020} &  18.55 &  29.03 &  33.06 &  20.97 &  20.16 &  18.55 &  25.81 &  23.39 &  25.0 &  12.9 &  16.13 &  22.14 \\
%         Pace Pred. \cite{wang2020selfsupervised} &  29.84 &  40.32 &  44.35 &  36.69 &  34.68 &  37.5 &  37.1 &  \textbf{46.77} &  35.89 &  22.18 &  24.19 &  35.41 \\
%         \hline
%         WildGait \textbf{(ours)} & \textbf{49.19} &  \textbf{52.42} &  \textbf{52.42} &  \textbf{49.19} &  \textbf{40.32} &  \textbf{50.81} &  \textbf{46.77} & \textbf{ 46.77} & \textbf{ 39.52} &  \textbf{37.1} &  \textbf{31.45} &  \textbf{45.09} \\
%     \end{tabular}}
%     \caption{Experiment C.}
%     \label{tab:unsupervised-casia-bag}
% \end{table*}
% }
% \begin{comment}
% \setlength{\tabcolsep}{0.8em}
% {\renewcommand{\arraystretch}{1.2}
% \begin{table}[hbt!]
%     % \resizebox{\textwidth}{!}{
%     \centering
%         \resizebox{\linewidth}{!}{
%         \begin{tabular}{l | rrrrr}
%          \toprule
%          \textbf{Method} &     WS &     CB &     CL &    CBG &    ALL \\
%          \midrule
%           Pretrain Kinetics &  24.00 &  \textbf{54.55} &  28.63 &  43.16 &  22.33 \\
%           \hline
%           Predict \& Cluster  &  33.47 &  35.69 &  20.51 &  36.32 &  34.13 \\
%           \hline
%           MS$^2$L &  42.88 &  38.43 &  27.78 &  49.57 &  40.87 \\
%           Pace Pred. &  44.15 &  37.84 &  25.00 &  51.28 &  43.72 \\
%           \hline
%           WildGait \textbf{(ours)} &  \textbf{63.84} &  48.63 &  \textbf{34.62} &  \textbf{67.09} &  \textbf{64.29} \\
%         \bottomrule
%         \end{tabular}}
%     % }
%     \caption{Transfer learning comparison with other unsupervised skeleton-based training methods. {\color{red} TODO re-evaluate kinetics}}
%     \label{tab:unsupervised-fvg}
% \end{table}
% }
% \end{comment}



==> sections/tabels/unsupervised.tex <==
\setlength{\tabcolsep}{0.8em}
{\renewcommand{\arraystretch}{1.2}
\begin{table*}[hbt!]
    \resizebox{\textwidth}{!}{
    \centering
    \begin{tabular}{l | ccccccccccc | c }
    \toprule
        & \multicolumn{12}{ c| }{\textbf{CASIA-B - Normal Walking}}\\
         &  0$^{\circ}$  &    18$^{\circ}$  &    36$^{\circ}$  &    54$^{\circ}$  &    72$^{\circ}$  &    90$^{\circ}$  &    108$^{\circ}$ &    126$^{\circ}$ &   144$^{\circ}$ &    162$^{\circ}$ &    180$^{\circ}$ & Mean \\
        \midrule
        Pretrained Kinetics  & 19.35 &  19.35 &  27.42 &  29.03 &  25.81 &  38.71 &  27.42 &  27.42 &  20.97 &  12.9 &  6.45 &  23.17 \\
        \hline
        Predict \& Cluster & 41.93 &  45.16 &  45.96 &  34.67 &  20.16 &  11.29 &  30.64 &  32.25 &  21.77 &  19.35 &  12.09 &  28.66 \\
        \hline
        MS$^2$L & 37.90 &  39.51 &  40.32 &  51.61 &  24.19 &  17.74 &  25.80 &  46.74 &  40.32 &  33.06 &  34.67 &  35.62 \\
        Pace Prediction  & 43.34 &  39.51 &  50.00 &  54.03 &  38.70 &  62.90 &  \textbf{70.96} & 70.16 &  54.03 &  66.93 &  64.51 &  55.91\\
        \hline
        WildGait \textbf{(ours)} & \textbf{72.58} &  \textbf{84.67} &  \textbf{90.32} &  \textbf{83.87} &  \textbf{63.70} &  \textbf{62.90} &  66.12 &  \textbf{83.06} &  \textbf{86.29} &  \textbf{84.67} &  \textbf{83.06} &  \textbf{78.29} \\
    \end{tabular}}
    \vspace{-2mm}
    \caption{Transfer learning comparison with other unsupervised skeleton-based training methods on CASIA-B. We report accuracy where the gallery set contains all viewpoints except the probe angle (top row).} 
    \label{tab:unsupervised-casia}
\end{table*}
}
